Clusters of primordial black holes

The Primordial Black Holes (PBHs) are gradually involved into consideration as the phenomenon having reliable basis. We discuss here the possibility of their agglomeration into clusters that may have several prominent observable features. The clusters can form due to closed domain walls appearance in the natural and the hybrid inflation with subsequent evolution and gravitational collapse. Early dustlike stages of dominance of heavy metastable dissipative particles, at which star-like objects are formed, can also naturally lead to formation of black hole clusters, remaining in the Universe after decay of particles, from which they have originated. The dynamical evolution of such clusters discussed here is of the crucial importance. Such a model inherits all the advantages of the single PBHs like possible explanation of existence of supermassive black holes (origin of the early quasars), binary BH merges registered by LIGO/Virgo through gravitational waves, contribution to reionization of the Universe, but also has additional benefits. The cluster could alleviate or completely avoid existing constraints on the single PBH abundance making PBHs a real dark matter candidate. The most of existing constraints on (single) PBH density should be re-considered as applied to the clusters. Also unidentified cosmic gamma-ray point-like sources could be (partially) accounted for by them. One can conclude, that it seems really to be much more viable model with respect to the single PBHs.

==> Dynamics/Dynamics.tex <==
Исследование гравитационной динамики скопления ПЧД после отцепления сводится к задаче об эволюции $N$-тел и может решаться только численно. Для этих целей мы использовали программный пакет \texttt{NBODY6++} \cite{2015MNRAS.450.4070W}, предназначенный для моделирования эволюции шаровых звёздных скоплений, с  % путем прямого интегрирования задачи $N$ тел. % На расстояниях, существенно превышающих гравитационные радиусы ПЧД, нет принципиальных различий между динамикой звёзд и ПЧД, что открывает возможность использования <<ядра>> пакета \texttt{NBODY6++}.
% с реализованными алгоритмами и методами, которые позволяют значительно оптимизировать вычисления.
рядом изменений: все разыгрываемые тела были лишены характеристик, определяющих их звёздную природу (светимость, тип звезд и их эволюция, металличность и т.д.), были переопределены <<размеры>> объектов в соответствии с массами ($r_i={r_g}_i=2GM_i/c^2$, где $r_g$~--- гравитационный радиус),
%(отметим, что в расчётах \texttt{NBODY6++} все тела считаются точечными, однако приписываемые <<размеры>> гравитирующих тел необходимы, чтобы определить условия слияния); 
был добавлен механизм слияния, в котором слияние двух ЧД происходит при их взаимном сближении на расстояние $r_{ij} \leq \varkappa ({r_g}_i+{r_g}_j)$, где коэффициент $\varkappa$ выбирался равным 3. 

Учитывая образующуюся плотную структуру центра скопления и множественность <<лёгких>> чёрных дыр \textbf{(см. рис. ??? или раздел ??? выше)}, вопрос о полностью корректном моделировании кластера остаётся открытым. Как видно из \textbf{рис. ???}, распределение маломассивной составляющей является почти однородным для всего кластера, а потому можно рассматривать её постоянным гравитирующим фоновым полем, в котором находится кластер, и, для простоты, исключить из непосредственного моделирования. При этом приближении удаётся проследить динамику <<массивной>> составляющей скопления с $M>0.1 M_\odot$. 

Рассмотрим характерный пример. При моделировании разыгрывалось $N=8600$ чёрных дыр в скоплении с массовым распределением
\begin{equation*}
	\frac{dN}{dM} \propto \frac{1}{M_\odot} \left(\frac{M_\odot}{M}\right)^\beta
\end{equation*}
и пространственным 
\begin{equation*}
	\rho(r)\propto r^{-\alpha},
\end{equation*}
которые при $\beta=2.4$ и $\alpha=2$ хорошо аппроксимируют центральные области кластера в диапазоне масс $10^{-1}\div10^{2} M_\odot$ \cite{2017JPhCS.934a2040N} \textbf{[Валера, уместна ли здесь эта ссылка????]}. Начальные скорости ПЧД моделировались в соответствии со средней скоростью ПЧД каждого пространственного слоя (см. раздел \ref{sec:detach}). \textbf{(ЕСТЬ ЛИ ТАМ УПОМИНАНИЕ О СКОРОСТЯХ?)}

\begin{figure}[t]
 \begin{center}
  \subfigure[Начальное (синее) и конечное (красное) массовые распределения ПЧД в кластере.]{
   \includegraphics[width=0.47\textwidth]{Dynamics/MassDist1.pdf}
   \label{fig:mass}
  }
  \subfigure[Изменение количества ПЧД в кластере со временем.]{
   \includegraphics[width=0.47\textwidth]{Dynamics/Num.pdf}
   \label{fig:num}
  }
 \end{center}
 \caption{Динамика кластера ПЧД до момента $z\sim20$. 
 Слева: изменение массового спектра. Справа: изменение общего количества ПЧД в кластере за счёт слияния и вылета.
 }
 \label{fig:Mass_Num_Evol}
\end{figure}

Результаты представлены на рис.~\ref{fig:Mass_Num_Evol}. Видно, что кластер, в целом, незначительно меняет свою структуру: массовый спектральный индекс не меняется ($\beta_\text{f}\approx 2.4$), количество частиц уменьшается на $\sim10\%$ (за счёт вылета и слияний ЧД). В результате слияний в кластере сохраняется доминирующая по массе центральная чёрная дыра. Интересно отметить, что наиболее интенсивно изменение числа ПЧД происходит в первые 50~млн. лет, в последующий период происходит выход на слабоменяющийся закон (см. рис.~\ref{fig:num}). Важно подчеркнуть, что кластер не разрушается и остаётся гравитационно связанной системой на момент $z\sim20$, когда, по оценкам, аккреция начинает оказывать существенное влияние на рост наиболее массивных чёрных дыр (см. \cite{2018Natur.553..473B}).

В литературе широко обсуждается проблема раннего образования галактик. Моделирование показывает, что раннее образование квазаров возможно в случае, если на момент $z\sim 20\div40$ уже существовали их ``зародыши''~--- либо объекты, в дальнейшем коллапсирующие в чёрные дыры (например, массивные плотные облака газа), либо непосредственно чёрные дыры с массами, доходящими до $10^5M_\odot$ (такая масса необходима для получения на $z\sim6$ массы квазара $M\sim10^9M_\odot$, см. \cite{...}). Однако возникновение на столь ранних красных смещениях массивных объектов требует дополнительного объяснения и является, в свою очередь, ничуть не меньшей проблемой, чем само существование ранних квазаров \cite{...}. Наш анализ показывает, что мы можем предложить ещё один сценарий естественного образования ``зародышей'' кластеров. 


==> biberosh.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ВСЕ ССЫЛКИ ПЕРЕНЕСЕНЫ В bib2.bib %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{thebibliography}{99}

%\bibitem{dub17} Rubin S. G., Khlopov M. Yu., Sakharov A. S. Primordial Black Holes from Non-Equilibrium Second Order Phase Transition //  Grav. Cosmol. S. 2000. Vol.  S6. P. 51-58.  arXiv:hep-ph/0005271.

%\bibitem{Ru2} Rubin S. G., Sakharov A. S. and Khlopov M. Y. The Formation of Primary Galactic Nuclei during Phase Transitions in the Early Universe //   J. Exp. Theor. Phys. 2001. Vol. 92. P. 921-929.

%\bibitem{Ru2a}  Khlopov M. Yu.,  Rubin S. G. and  Sakharov A. S. Primordial Structure of Massive Black Hole Clusters //  Astroparticle Physics. 2005. Vol. 23. P. 265-277. arXiv:astro-ph/0401532.

%\bibitem{DokEroRub05} Dokuchaev V., Eroshenko Yu., Rubin S. Quasars formation around clusters of primordial black holes //  Grav. Cosmol. 2005. Vol. 11. P. 99-104. arXiv:astro-ph/0412418.

%\bibitem{KolTka94} Kolb E.~W. and Tkachev I.~I. Large Amplitude Isothermal Fluctuations And High Density Dark Matter Clumps //  Phys. Rev. D. 1994. Vol. 50. P. 769.  [arXiv:astro-ph/9403011]. 

%%%

%\bibitem{DokEroRub09} V.I. Dokuchaev, Yu.N. Eroshenko, S.G. Rubin, ``Gravitational Wave Bursts from Collisions of Primordial Black Holes in Clusters'', Astronomy Letters, Vol. 35, p. 143 (2009); arXiv:1003.4158 [astro-ph.CO].

%\bibitem{lisa11} V.I. Dokuchaev, Yu.N. Eroshenko, S.G. Rubin, ``Early formation of galaxies initiated by clusters of primordial black holes'', Astron. Rep. 52, 779 (2008); arXiv:0801.0885 [astro-ph].

%\bibitem{lisa12} Mouri H.,  Taniguchi Y. Runaway Merging of Black Holes: Analytical Constraint on the Timescale //    Astrophys. J. 2002. Vol. 566. P. L17-L20. arXiv:astro-ph/0201102.

%\bibitem{lisa15} Will C. M. On the Rate of Detectability of Intermediate-Mass Black Hole Binaries Using LISA //    Astrophys. J. 2004. Vol. 611. P. 1080-1083. arXiv:astro-ph/0403644.

%\bibitem{lisa17} Sesana A. et al. The Gravitational Wave Signal from Massive Black Hole Binaries and Its Contribution to the LISA Data Stream //    Astrophys. J. 2005. Vol. 623. P. 23-30. 	arXiv:astro-ph/0409255.

%%%

%\bibitem{p41} Ya. B. Zel'dovich and I. D. Novikov, Sov. Astron. 10, 602 (1967).

%\bibitem{p22} S. Hawking, Mon. Not. R. Astron. Soc. 15, 75 (1971).

%\bibitem{p24} A. S. Josan, A. M. Green, and K. A. Malik, Phys. Rev. D 79, 103520 (2009).

% \bibitem{p11} B. J. Carr, Astrophys. J. 201, 1 (1975).

%\bibitem{p25} M. Yu. Khlopov and A. G. Polnarev, Phys. Lett. B 97, 383 (1980).

%\bibitem{p40} N. A. Zabotin, P. D. Nasel'skii, and A. G. Polnarev, Sov. Astron. 31, 353 (1987).

%\bibitem{p4} V. A. Berezin, V. A. Kuzmin, and I. I. Tkachev, Phys. Lett. B 120, 91 (1983).

%\bibitem{p26} M. Yu. Khlopov, R. V. Konoplich, S. G. Rubin, and A. S. Sakharov, Preprint 1203 (I Roma University, 1998); arXiv:hep-ph/9807343.

%\bibitem{p37} S. G. Rubin, M. Yu. Khlopov, and A. S. Sakharov, Grav. Cosmol. S 6, 51 (2000).

% \bibitem{DolSil93} A. Dolgov and J. Silk, ``Baryon isocurvature fluctuations at small scales and baryonic dark matter'', Phys. Rev. D 47, 4244 (1993).

% \bibitem{Dol18} Dolgov A D, ``Massive and supermassive black holes in the contemporary and early Universe and problems in cosmology and astrophysics'', Phys. Usp. 61 (2) (2018).

% \bibitem{p23} P. Ivanov, P. Naselsky, and I. Novikov, Phys. Rev. D 50, 7173 (1994).

%\end{thebibliography}
